A Model-Based Testing Tool for Asynchronous Reactive Systems

Reactive systems are characterized by the interaction with the environment, where the exchange of the input and output stimuli, usually, occurs asynchronously. Systems of this nature, in general, require a rigorous testing activity over their developing process. Therefore model-based testing has been successfully applied over asynchronous reactive systems using Input Output Labeled Transition Systems (IOLTSs) as the basis. In this work we present a reactive testing tool to check conformance, generate test suites and run test cases using IOLTS models. Our tool can check whether the behavior of an implementation under test (IUT) complies with the behavior of its respective specification. We have implemented a classical conformance relation \ioco and a more general notion of conformance based on regular languages. Further, the tool provides a test suite generation in a black-box testing setting for finding faults over IUTs according to a specific domain. We have also described some case studies to probe the tool's functionalities and also to highlight a comparative analysis on both conformance approaches. Finally, we offer experiments to evaluate the performance of our tool using several scenarios.

==> figs/fig-tool.tex <==
\begin{figure}[hbt]
%	\vspace*{-2ex}
	\centering
	\includegraphics[scale=0.35]{figs/arquiteturaFerramenta.png}
	\caption{Tool's Architecture}
	\label{fig:arquiteturaFerramenta}
	\vspace*{-3ex}
\end{figure} 

